Joint Communication and Control: Causal Coordination Coding for Witsenhausen Counterexample

In decentralized network control, communication plays a crucial role by transforming local observations into shared knowledge, enabling agents to coordinate their actions. This paper investigates how communication facilitates cooperation behavior and therefore improves the overall performance in Witsenhausen counterexample, a canonical toy problem in distributed decision-making. We consider the vector-valued setups where the encoder, i.e., the first decision-maker (DM) acts causally and the decoder, i.e., the second DM, operates noncausally, 1) without and 2) with access to channel feedback. Using a coordination coding framework, we characterize the achievable power-estimation cost regions in single-letter expressions for both scenarios. We show that feedback enlarges the coordination region compared with the no-feedback setup. Building on the characterization of the power-estimation cost region, we propose a hybrid strategy that combines discrete quantization with a continuous Gaussian codebook, the Zero Estimation Cost (ZEC) strategy. This strategy uses coding tools that allow perfect reconstruction of the target symbols, leading to an asymptotic estimation cost equal to zero, while substantially reducing the power cost. Moreover, when channel feedback is available, we propose an analogous ZEC strategy that simultaneously achieves zero power and zero estimation costs in the low-noise regime. Finally, we establish that, when restricted to jointly Gaussian random variables, the performance is identical across all setups featuring at least one causal DM, regardless of the presence of feedback information.

==> sections/Non_ZEC_2.tex <==
In this section, we apply a test channel between the aux. RV $W_2$ and the source state $X_0$ with a cross-over probability $\gamma$. Given nonnegative parameters $V_1,a,\gamma$, we consider
% \vspace{-0.1cm}
\begin{align}
\left|
\begin{aligned}
    &X_0\sim\mathcal{N}(0,Q),\\
    & W_1\sim\mathcal{N}(0, V_1),\\
    % \text{(coefficient $a$ needs to be revealed to $U_1$)}\\
    & W_2=\left\{
          \begin{aligned}
              & a\cdot S &\text{with probability }1-\gamma,\\
              & -a\cdot S&\text{with probability }\gamma,
          \end{aligned}   
        \right.\\
        &\quad\quad\quad  \text{ where } S=\mathsf{sign}(X_0),\\
    & U_1 = W_1 + a\cdot S - X_0,\\
    & X_1 = U_1+X_0 = W_1 + a\cdot S, \\
    & Y_1 = X_1 + Z_1 = W_1 + a\cdot S+ Z_1,\quad Z_1\sim\mathcal{N}(0,N).
\end{aligned}
\right. 
\label{eq: lossy system}
\end{align}

% \vspace{-0.1cm}
The design of $W_2$ as a binary RV dependent on $X_0$ rather than a deterministic variable introduces additional randomness, which affects the estimation precision of $X_1$ from $(W_1,W_2,Y_1)$. Note that, if $\gamma=0$ or $1$, the above system degrades to a deterministic relation, where $X_1=W_1+W_2$ or $X_1=W_1-W_2$, respectively. In either case, the estimation cost is zero, hence we recover the ZEC scheme. Furthermore, it can be easily shown that the \ac{mmse} remains the same for $\gamma$ and $1-\gamma$. Therefore, we can restrict our analysis to $\gamma\in[0,0.5]$, without loss of generality.


To simplify the presentation of the estimation cost result presented in Theorem \ref{thm: coord_2_testch}, we define the following quantities:
\begin{align*}
     &G_0(w_1) =\frac{1}{\sqrt{V_1}}\phi\brackets{\frac{w_1}{\sqrt{V_1}}},\\
     &G_1(w_1,y_1) = \frac{1}{\sqrt{N}}\phi\brackets{\frac{y_1-(w_1+a)}{\sqrt{N}}},\\
     &G_2(w_1,y_1) = \frac{1}{\sqrt{N}}\phi\brackets{\frac{y_1-(w_1-a)}{\sqrt{N}}},\\
     &I(w_1,y_1)\!=\!G_0\!\sbrackets{\frac{ [(1-\gamma)G_1 - \gamma G_2]^2}{(1-\gamma)G_1 + \gamma G_2}\! +\! \frac{ [\gamma G_1 - (1-\gamma) G_2]^2}{\gamma G_1 + (1-\gamma) G_2}}.
\end{align*}
Similarly, we define the set of admissible parameters
\begin{align}
    \!\mathcal{A}^\gamma(P)&\! =\! \{a\geq 0:h(Y_1)+H_2(\gamma) - h(Y_1|W_1,W_2)\geq 1,\nonumber \\
    &\quad \text{and } V_1 = P-\brackets{Q+a^2-2a\sqrt{\frac{2Q}{\pi}}}\geq 0\}, \label{eq: admissible set lossy}
\end{align}
where $h(Y_1)$ is the entropy calculated from the distribution defined in \eqref{eq: Y_1 distr}, $H_2(\gamma)=-\gamma \log_2(\gamma)-(1-\gamma)\log_2(1-\gamma)$ is a binary entropy, and $h(Y_1|W_1,W_2)$ is the following Gaussian mixture differential entropy
\begin{align*}
    h\brackets{(1-\gamma) \frac{1}{\sqrt{N}}\phi\brackets{\frac{y-a}{\sqrt{N}}} + \gamma \frac{1}{\sqrt{N}}\phi\brackets{\frac{y+a}{\sqrt{N}}}}.
\end{align*}

By setting $\gamma=0$ (and also $\gamma=1$), \eqref{eq: admissible set lossy} recovers the admissible parameter set $\mathcal{A}^0(P)$ given in \eqref{eq: admissible set} of the ZEC scheme. Therefore,
\begin{align}
    \mathcal{A}^0 (P) \subseteq \mathcal{A}^\gamma (P),
\end{align}
indicating that the Non-ZEC scheme permits lower power costs compared to the ZEC scheme.


The full proof using the above quantities is provided in the appendix[]. Additionally, the derivation of the ZEC cost function sketched in equations \eqref{eq: coord2 power cost constraint} to \eqref{eq: admissible set} can also be seen as a special case of the derivation of the Non-ZEC scheme by setting $\gamma = 0$.

 \begin{theorem}\label{thm: coord_2_testch}
    Given $P\geq P_2^{\min}$, the optimal estimation cost induced by the Non-ZEC scheme \eqref{eq: lossy system} is given by
    \begin{align}
         S_{\mathsf{Non}\text{-}\mathsf{ZEC}}(P)= \min_{a\in\mathcal{A}^\gamma(P),\gamma\in[0,0.5]}\quad\big\{F(a,\gamma,P)\big\},\label{eq: cost func lossy}
         \end{align}
where,
         \begin{align}
         F(a,\gamma,P)=a^2 -\frac{a^2}{2}\iint I(w_1,y_1) dw_1dy_1. \label{eq: F(a,gamma,P)}
    \end{align}
    
\end{theorem}

In this theorem, $F(a,\gamma,P)$ represents the achievable estimation cost for a given pair $(a,\gamma)$ at the power budget $P\geq P_2^{\min}$, and we can minimize $F$ over all admissible parameters $a\in\mathcal{A}^\gamma(P),\gamma\in[0,0.5]$ to get the optimized result \eqref{eq: cost func lossy}. Moreover, by plugging in $\gamma=0$, $S_{\mathsf{Non}\text{-}\mathsf{ZEC}}(P)$ boils down to $S_{\mathsf{ZEC}}(P) = 0$ when $P\geq P^*$ given in \eqref{eq: P^*}.


\begin{figure}[h]
        \centering
        \input{fig/different_gamma}
        \caption{Evolution of $F(a,\gamma,P)$ with different values of $\gamma=0,0.05, 0.1,0.5$. When $\gamma=0$, $F(a,0,P) = S_{\mathsf{ZEC}}(P)$ in \eqref{eq: cost function lossless}, and when $\gamma=0.5$, the lower boundary of $F(a,0.5,P)$ recovers that of the two-point strategy (yellow dashed curve).}
        \label{fig: diff gamma}
    \end{figure}


To analyze the performance of the Non-ZEC scheme, we examine how different values of $\gamma\in[0,0.5]$ affect its achievable cost region. Figure \ref{fig: diff gamma} illustrates the function $F(a,\gamma,P)$ in \eqref{eq: F(a,gamma,P)} by plotting \textit{all} the admissible points $a\in\mathcal{A}^\gamma(P)$ at each $P\geq P_2^{\min}$, resulting in a 2-dimensional region, for fixed parameters of $\gamma\in \{0,0.01,0.1,0.5\}$ compared to the original two-point strategy at $Q=1,N=0.15$. 


 
As shown in Figure \ref{fig: diff gamma}, $F(a,0,P)$ aligns with the ZEC cost function $S_{\mathsf{ZEC}}(P)$ in \eqref{eq: cost function lossless}, as expected. Gradually increasing  $\gamma$, which introduces more randomness in $W_2$, allows for a reduction in power cost at the expense of sacrificing estimation accuracy. Ultimately, when  $\gamma=0.5$, which means $W_2$ provides no information about the source $X_0$ at all, the required power budget reaches its minimum, and the lower boundary of the achievable cost $F(a,0.5,P)$ aligns with that of the original two-point strategy. 


\begin{figure}[t]
        \centering      \input{fig/Q=1,N=0.15,Non_ZEC}
        \caption{Comparison of the four closed-form cost functions $S_{\mathsf{Non}\text{-}\mathsf{ZEC}}(P)$, $S_2(P)$, $S_\ell(P)$, $S_{\mathsf{G}}(P)$, and the induced time-sharing cost $S_{\mathsf{t}\text{-}\mathsf{s}}(P)$ at $Q=1,N=0.15$. }
        \label{fig:Q=1,N=0.15,lossy}
    \end{figure}


In Figure \ref{fig:Q=1,N=0.15,lossy}, We plot the optimized achievable estimation cost function $S_{\mathsf{Non}\text{-}\mathsf{ZEC}}(P)$ in \eqref{eq: cost func lossy} and compare it with the other three cost functions $S_2(P), S_\ell(P)$ and $S_{\mathsf{G}}(P)$. The numerical results indicate that the Non-ZEC scheme functions effectively as a time-sharing mechanism between the ZEC scheme and the original two-point strategy. Moreover, $S_{\mathsf{t}\text{-}\mathsf{s}}(P)$ represents the estimation cost resulting from the time-sharing operation between the optimal Gaussian strategy $S_{\mathsf{G}}(P)$ and the ZEC strategy $S_{\mathsf{ZEC}}(P)$, which in this scenario, is shown to be superior to the Non-ZEC scheme.


==> sections/Proof_of_Non_ZEC_Theorem.tex <==
The information constraint \eqref{info result} can be reformulated as
    \begin{align}
        &I(W_1,W_2;Y_1) - I(W_2;X_0|W_1)\nonumber\\
    &= h(Y_1)+h(W_2|X_0,W_1) - h(Y_1|W_1,W_2)-h(W_2)\label{app info constraint 1}\\
    &= h(Y_1)+h(W|X_0,W_1) - h(Y_1|W_1,W_2)-h(W), \label{app info constraint 2}
    \end{align}
   where step \eqref{app info constraint 1} follows from the chain rule of mutual information, and in step \eqref{app info constraint 2}, we use the substitution:
    \begin{align*}
        W=W_2/a\sim\left\{
          \begin{aligned}
              & S &\text{with probability }1-\gamma,\\
              & -S&\text{with probability }\gamma,
          \end{aligned}   
        \right.
    \end{align*}
   with $S = \mathsf{sign}(X_0)$, a discrete random variable. Furthermore, by the scaling property of differential entropy, i.e., $h(cX) = h(X) + \log |c|$ for a constant $c \ne 0$, the constant $\log|a|$ that appears in both $h(W_2|X_0, W_1)$ and $h(W_2)$ cancels out, which justifies the equivalence between \eqref{app info constraint 1} and \eqref{app info constraint 2}.
 
Next, we examine each entropy term involved in \eqref{app info constraint 2} respectively
\begin{itemize}
    \item $h(Y_1):$ Since $ Y_1 = W_1 + a\cdot S + Z_1$ and $W_1\indep Z_1$ are both Gaussian distributed, the conditional distribution is
\begin{align*}
    f_{Y_1|S}(y|s ) = \frac{1}{\sqrt{2\pi(V_1+N)}}\exp{\brackets{-\frac{(y-a\cdot s)^2}{2(V_1+N)}}}.
\end{align*}
Moreover, since $\mathbb P(S=-1) = \mathbb P(S=+1) = \frac{1}{2}$, we have 
\begin{align}
    &f_{Y_1}(y)\\
    &= \sum_{s\in\{-1,+1\}}f_{Y_1|S}(y|s )\mathbb P(s)\nonumber\\
    &=\frac{1}{2\sqrt{(V_1+N)}}\brackets{\phi\brackets{\frac{y-a}{\sqrt{V_1+N}}}+ \phi\brackets{\frac{y+a}{\sqrt{V_1+N}}}},\label{eq: term 1}
\end{align}
according to which we can calculate $h(Y_1)$.
\item $h(W|X_0,W_1)$: Since $W$ is independent of $W_1=w_1$ once $X_0=x_0$ is given, we have
\begin{align*}
    W|X_0=x_0,W_1=w_1\sim \left\{
          \begin{aligned}
              & s &\text{with probability }1-\gamma,\\
              & -s&\text{with probability }\gamma,
          \end{aligned}   
        \right.
\end{align*}
where $s = \mathsf{sign}(x_0)$. This defines a binary discrete distribution. Thus, $h(W|X_0,W_1)$ is a binary entropy that takes the following form
\begin{align}
    h(W|X_0,W_1)
    = -\sbrackets{(1-\gamma)\log_2(1-\gamma) + \gamma \log_2\gamma}.\label{eq: term 2}
\end{align}
\item $h(Y_1|W_1,W_2)$: Because 
\begin{align*}
    h(Y_1|W_1,W_2)
    &= h(W_1 + a\cdot S+Z_1|W_1,W_2)\\
    &=h( a\cdot S+Z_1|W_2).
\end{align*}
The conditional distribution takes the following form
\begin{align*}
    &aS+Z_1|W_2 = a\sim \left\{
          \begin{aligned}
              & a+Z_1 &\text{with probability }1-\gamma,\\
              & -a+Z_1&\text{with probability }\gamma.
          \end{aligned}   
        \right.
\end{align*}
Moreover, since $Z_1\sim\mathcal{N}(0,N)$ is the independent additive noise, 
\begin{align*}
    &f(a\cdot S+Z_1|W_2=a)\\
    &=(1-\gamma) \frac{1}{\sqrt{N}}\phi\brackets{\frac{y-a}{\sqrt{N}}} + \gamma \frac{1}{\sqrt{N}}\phi\brackets{\frac{y+a}{\sqrt{N}}},
\end{align*}
is also a Gaussian mixture distribution.

And similarly,
\begin{align*}
    &f(a\cdot S+Z_1|W_2=-a)\\
    &=\gamma \frac{1}{\sqrt{N}}\phi\brackets{\frac{y-a}{\sqrt{N}}} + (1-\gamma) \frac{1}{\sqrt{N}}\phi\brackets{\frac{y+a}{\sqrt{N}}}.
\end{align*}
We can see that the above two Gaussian mixture distributions are just swapped mixture weights and the shape of one is just “mirrored” left-to-right of the other one. Hence, the differential entropy (which is shift-invariant in the sense of mixing) remains the same. Therefore,
\begin{align}
    &h(a\cdot sign(X_0)+Z_1|W_2)\nonumber\\
    &=\frac{1}{2}h(a\cdot sign(X_0)+Z_1|W_2=a)\nonumber \\
    &\quad + \frac{1}{2}h(a\cdot sign(X_0)+Z_1|W_2=-a) \nonumber\\
    &=h(a\cdot sign(X_0)+Z_1|W_2=a)\nonumber\\
    &=h\brackets{(1-\gamma) \frac{1}{\sqrt{N}}\phi\brackets{\frac{y-a}{\sqrt{N}}} + \gamma \frac{1}{\sqrt{N}}\phi\brackets{\frac{y+a}{\sqrt{N}}}}.\label{eq: term 3}
\end{align}

\item $h(W)$: Since the marginal $\mathbb P(W=1) = \mathbb P(W=-1) = \frac{1}{2}$, we obtain that
\begin{align}
    h(W)=1.\label{eq: term 4}
\end{align}

\end{itemize}


Given the above results \eqref{eq: term 1} - \eqref{eq: term 4} for calculating the information constraint, together with the power constraint, same as in \eqref{eq: coord2 power cost constraint}, the admissible set is given by
\begin{align*}
    \!\mathcal{A}^\gamma(P)&\! =\! \{a\geq 0:h(Y_1)+H_2(\gamma) - h(Y_1|W_1,W_2)\geq 1,\nonumber \\
    &\quad \text{and } V_1 = P-\brackets{Q+a^2-2a\sqrt{\frac{2Q}{\pi}}}\geq 0\}, 
\end{align*}
as provided in \eqref{eq: admissible set lossy}.

Next, given $\gamma\in[0,0.5],P\geq 0$, and for a feasible parameter $a\in\mathcal{A}^\gamma (P)$, we are interested in deriving the \ac{mmse} estimator of $X_1$ given $W_1=w_1,W_2=w_2,Y_1=y_1$, namely,
\begin{align*}
    \mathbb E[X_1|w_1,w_2,y_1] = \int x_1 f(x_1|w_1,w_2,y_1) dx_1.
\end{align*}
Hence, we need the closed-form expression of the following conditional probability distribution:
\begin{align*}
    \mathbb P(x_1|w_1,w_2,y_1)&= \mathbb P(w_1+a\cdot s|w_1,w_2,y_1)\\
    &= \mathbb P(s|w_1,w_2,y_1),
\end{align*}
which reduces to a two-point distribution. Since
\begin{align}
    &\mathbb P(s=1|w_1,w_2,y_1)\nonumber\\
    &=\frac{\mathbb P(s=1,w_2,y_1|w_1)}{\mathbb P(w_2,y_1|w_1)}\nonumber\\
     &=\frac{\mathbb P(w_2,y_1|w_1,s=1)\mathbb P(s=1|w_1)}{\sum_{s'\in\{-1,1\}} \mathbb P(w_2,y_1|w_1,s')\mathbb P(s'|w_1)}\nonumber\\
    &=\frac{\mathbb P(w_2,y_1|w_1,s=1)\mathbb P(s=1)}{\sum_{s'\in\{-1,1\}} \mathbb P(w_2,y_1|w_1,s')\mathbb P(s')}\nonumber\\
    &=\frac{\frac{1}{2}\mathbb P(w_2,y_1|w_1,s=1)}{\sum_{s'\in\{-1,1\}}\frac{1}{2} \mathbb P(w_2,y_1|w_1,s')}\nonumber\\
    &=\frac{\mathbb P(w_2,y_1|w_1,s=1)}{\sum_{s'\in\{-1,1\}}\mathbb P(w_2,y_1|w_1,s')}\nonumber\\
    &= \frac{\mathbb P(y_1|w_1,s=1)\cdot\mathbb P(w_2|s=1,w_1,y_1)}{\sum_{s'\in\{-1,1\}}\mathbb P(w_2,y_1|w_1,s')}   \label{eq: prob coord-2 text channel}
\end{align}
Since $Y_1 = W_1+a\cdot S + Z_1$, the term $\mathbb P(y_1|w_1,s=1)$ above becomes a Gaussian distribution
\begin{align*}
    \mathbb P(y_1|w_1,s=1) = \frac{1}{\sqrt{N}}\phi\brackets{\frac{y_1-(w_1+a)}{\sqrt{N}}}\triangleq G_1.
\end{align*}
 Moreover, because of the Markov chain $W_2-\!\!\!\!\minuso\!\!\!\!- S    -\!\!\!\!\minuso\!\!\!\!- (W_1, Y_1)$, we obtain
\begin{align*}
   \mathbb P(w_2|s=1,w_1,y_1) = \mathbb P(w_2|s=1) .
\end{align*}
Therefore, \eqref{eq: prob coord-2 text channel} becomes
\begin{align*}
   \mathbb P(s=1|w_1,w_2,y_1)
    =\frac{\mathbb P(w_2|s=1)G_1}{\mathbb P(w_2|s=1)G_1 + \mathbb P(w_2|s=-1)G_2}.
\end{align*}
where $G_2\triangleq \frac{1}{\sqrt{N}}\phi\brackets{\frac{y_1-(w_1-a)}{\sqrt{N}}}$.

Therefore, 
\begin{align*}
    \mathbb P(s=-1|w_1,w_2,y_1)
    &= 1-\frac{\mathbb P(w_2|s=1)G_1}{\mathbb P(w_2|s=1)G_1 + \mathbb P(w_2|s=-1)G_2}\\
    &= \frac{\mathbb P(w_2|s=-1)G_2}{\mathbb P(w_2|s=1)G_1 + \mathbb P(w_2|s=-1)G_2}.
\end{align*}
This means, 
\begin{align*}
    &\mathbb P(x_1=w_1+a|w_1,w_2,y_1)
    = \frac{\mathbb P(w_2|s=1)G_1}{\mathbb P(w_2|s=1)G_1 + \mathbb P(w_2|s=-1)G_2},\\
    &\mathbb P(x_1=w_1-a|w_1,w_2,y_1) 
    = \frac{\mathbb P(w_2|s=-1)G_2}{\mathbb P(w_2|s=1)G_1 + \mathbb P(w_2|s=-1)G_2}.\label{eq: distr x_1=w_1-a}
\end{align*}
Hence, when $w_2=a$, the MMSE estimator is
\begin{align*}
    &\mathbb E[X_1|W_1=w_1,W_2=a,Y_1=y_1] \\
    &=w_1 + \frac{ \mathbb P(w_2=a|s=1)G_1 - \mathbb P(w_2=a|s=-1) G_2}{ \mathbb P(w_2=a|s=1)G_1 +  \mathbb P(w_2=a|s=-1) G_2}\cdot a\\
    &=w_1 + \frac{ (1-\gamma)G_1 - \gamma G_2}{(1-\gamma)G_1 + \gamma G_2}\cdot a.
\end{align*}
And on the other hand, when $w_2=-a$,
\begin{align*}
    &\mathbb E[X_1|W_1=w_1,W_2=-a,Y_1=y_1] \\
    &=w_1 + \frac{ \mathbb P(w_2=-a|s=1)G_1 - \mathbb P(w_2=-a|s=-1)G_2}{ \mathbb P(w_2=-a|s=1)G_1 +  \mathbb P(w_2=-a|s=-1) G_2}\cdot a\\
    &=w_1 + \frac{ \gamma G_1 - (1-\gamma) G_2}{\gamma G_1 + (1-\gamma) G_2}\cdot a.
\end{align*}
And the joint distribution of $(w_1,w_2,y_1)$ when $w_2=a$ is
\begin{align*}
    &\mathbb P(w_1,w_2=a,y_1)\\
    &=f(w_1)\cdot \mathbb P(a,y_1|w_1) \\
    &=f(w_1)\brackets{\sum_{s'\in\{-1,1\}} \mathbb P(a,y_1|w_1,s')\mathbb P(s')}\\
    &=\frac{f(w_1)}{2}\brackets{\sum_{s'\in\{-1,1\}} \mathbb P(y_1|w_1,s')\cdot\mathbb P(a|s')}\\
    &=\frac{G_0}{2}\sbrackets{(1-\gamma)G_1 + \gamma G_2} ,
\end{align*}
where $G_0\triangleq \frac{1}{\sqrt{V_1}}\phi\brackets{\frac{w_1}{\sqrt{V_1}}}$. Similarly, if we plug in $w_2=-a$, we get
\begin{align*}
     \mathbb P(w_1,w_2=-a,y_1) =\frac{G_0}{2}\sbrackets{\gamma G_1 + (1-\gamma) G_2} .
\end{align*}
Next, we calculate the expected squared MMSE estimation in the following way:
\begin{align}
    &\mathbb{E}\sbrackets{\left(\mathbb{E}\sbrackets{X_1|W_1,W_2,Y_1}\right)^2} \\
    &=\iiint (\mathbb E[X_1|w_1,w_2,y_1])^2\mathbb P(w_1,w_2,y_1) dw_1dw_2dy_1\nonumber\\
    &=\sum_{w_2\in\{a,-a\}}\iint (\mathbb E[X_1|w_1,w_2,y_1])^2\mathbb P(w_1,w_2,y_1) dw_1dy_1\nonumber\\
    &=\iint (\mathbb E[X_1|w_1,w_2=a,y_1])^2\mathbb P(w_1,w_2=a,y_1) dw_1dy_1 \nonumber \\
    &\quad + \iint (\mathbb E[X_1|w_1,w_2=-a,y_1])^2\mathbb P(w_1,w_2=-a,y_1) dw_1dy_1\nonumber\\
    &=\iint w_1^2 \cdot \sbrackets{\mathbb P(w_1,w_2=a,y_1) + \mathbb P(w_1,w_2=-a,y_1)} dw_1dy_1\nonumber \\
    &\quad + a\iint G_0\sbrackets{(1-\gamma)G_1 - \gamma G_2}w_1dw_1dy_1\nonumber\\
    &\quad + a\iint G_0\sbrackets{\gamma G_1 - (1-\gamma) G_2}w_1dw_1dy_1\nonumber \\
    &\quad + \frac{a^2}{2}\iint I(w_1,y_1)dw_1dy_1\nonumber\\
    &= \mathbb E[W_1^2]+a\iint G_0\sbrackets{G_1 -  G_2}w_1dw_1dy_1\nonumber \\
    &\quad + \frac{a^2}{2}\iint I(w_1,y_1)dw_1dy_1.\label{eq: conditional exp}
\end{align}
The first term above boils down to $\mathbb E[W_1^2] = V_1$. Moreover, since
\begin{align*}
   &\iint G_0G_1w_1dw_1dy_1\\
    &=\iint \frac{1}{\sqrt{V_1}} \phi\brackets{\frac{w_1}{\sqrt{V_1}}}\frac{1}{\sqrt{N}} \phi\brackets{\frac{y_1-(w_1+a)}{\sqrt{N}}}w_1dw_1dy_1\\
    &=\int \frac{w_1}{\sqrt{V_1}} \phi\brackets{\frac{w_1}{\sqrt{V_1}}} \sbrackets{\int \frac{1}{\sqrt{N}} \phi\brackets{\frac{y_1-(w_1+a)}{\sqrt{N}}} dy_1}dw_1,
\end{align*}
where the inner integral is with regard to the distribution of $Y_1\sim\mathcal{N}(w_1+a,N)$ conditioned on $W_1=w_1$, therefore the integral value is actually a cumulative distribution with
\begin{align*}
    \int \frac{1}{\sqrt{N}} \phi\brackets{\frac{y_1-(w_1+a)}{\sqrt{N}}} dy_1=1,
\end{align*}
and in this way, the outer integral becomes
\begin{align*}
    \int \frac{w_1}{\sqrt{V_1}} \phi\brackets{\frac{w_1}{\sqrt{V_1}}} dw_1 = \mathbb E[W_1] = 0.
\end{align*}
As a result, we have
\begin{align*}
    \iint G_0G_1w_1dw_1dy_1 = 0.
\end{align*}
Similarly, we can obtain
\begin{align*}
    \iint G_0G_2w_1dw_1dy_1 = 0.
\end{align*}
Therefore, the term in \eqref{eq: conditional exp} becomes
\begin{align*}
   a\iint G_0\sbrackets{G_1 -  G_2}w_1dw_1dy_1 =0.
\end{align*}
Overall, the MMSE of estimating $X_1 = W_1+a\cdot S$ given $W_1,W_2,Y_1$ is 
\begin{align*}
    &\mathbb E[(X_1-\mathbb E[X_1|W_1,W_2,Y_1])^2]\\
    &= \mathbb{E}[X_1^2] - \mathbb{E}\sbrackets{\left(\mathbb{E}\sbrackets{X_1|W_1,W_2,Y_1}\right)^2}\\
    &=\mathbb E[(W_1+a\cdot S)^2] - \mathbb{E}\sbrackets{\left(\mathbb{E}\sbrackets{X_1|W_1,W_2,Y_1}\right)^2}\\
    &=V_1+a^2-\brackets{V_1  +\frac{a^2}{2}\iint I(w_1,y_1)dw_1dy_1}\\
    &=a^2 -\frac{a^2}{2}\iint I(w_1,y_1)dw_1dy_1.
\end{align*}
This concludes the proof of Theorem \ref{thm: coord_2_testch}. \hfill \qedsymbol{}

==> sections/optimal_Gaussian.tex <==
In order to investigate the region of achievable pairs of Witsenhausen costs $(P,S)$, we focus on its boundary. We fix the power cost to some parameter $P\geq 0$, and we investigate the optimal estimation cost at the decoder.
\begin{definition}
    Given a power cost parameter $P\geq 0$, the optimal estimation cost \emph{MMSE} is the solution of the optimization problem:
        \begin{align*}
            S(P) &= \inf_{\mathcal{P}\in\mathbb P(P)}\mathbb E[(X_1 - U_2)^2],\\
            \mathbb P(P) &= \{ (\mathcal{P}_{W_1},\mathcal{P}_{W_2|X_0 W_1},\mathcal{P}_{U_1|X_0 W_1},\mathcal{P}_{U_2|W_1 W_2 Y_1}):\\
            &\quad\quad \text{s.t. }P = \mathbb E_\mathcal{P}[U_1^2] \text{ and },\\
            &\quad\quad I(W_1,W_2;Y_1) - I(W_2;X_0|W_1)>0\}.
        \end{align*}

\end{definition}

Due to the usage of Mininum Mean Squared Error estimation cost, the decoder's optimal decision policy is well-known and given by the conditional expectation stated in the following lemma.
\begin{lemma}
    Given a power cost parameter $P\geq 0$, the optimal estimation cost \emph{MMSE} satisfies
        \begin{align}
            S^*(P) &= \inf_{\mathcal{P}\in\mathbb P_c(P)}\mathbb E[(X_1 - \mathbb E[X_1|W_1,W_2,Y_1])^2],\label{eq: opt prob}\\
            \mathbb P_c(P) &= \{ (\mathcal{P}_{W_1},\mathcal{P}_{W_2|X_0 W_1},\mathcal{P}_{U_1|X_0 W_1}):\nonumber\\
            &\quad\quad \text{s.t. }P = \mathbb E_\mathcal{P}[U_1^2],\nonumber\\
            &\quad\quad I(W_1,W_2;Y_1) - I(W_2;X_0|W_1)>0\}.\nonumber
        \end{align}
\end{lemma}

Note that the remaining optimization problem \eqref{eq: opt prob} is difficult to solve since the domain is the set of real-valued distributions. In the following, we investigate this optimization problem by considering additional assumptions on the set of random variables involved to be jointly Gaussian.

\begin{proposition}
    Given a power cost parameter $P\geq 0$, the estimation cost $S_{\mathsf {G}}(P)$ satisfies   
        \begin{align}
            &S_{\mathsf {G}}(P) = \inf_{\mathcal{P}\in\mathbb P_{\mathsf {G}}(P)}\mathbb E\Big[\big(X_1 - \mathbb E\big[X_1\big|W_1,W_2,Y_1\big]\big)^2\Big],\\
            &\mathbb P_{\mathsf {G}}(P) = \Bigl\{  (\mathcal{P}_{W_1},\mathcal{P}_{W_2|X_0, W_1},\mathcal{P}_{U_1|X_0, W_1})\quad \text{s.t. }P = \mathbb E\big[U_1^2\big],\nonumber\\
            &\quad I(W_1,W_2;Y_1) - I(W_2;X_0|W_1)\geq0,\text{ and }\label{eq: opt domain w/o feedback}\\
            &\quad X_0,W_1,W_2,U_1,X_1,Y_1,U_2\text{ are jointly Gaussian}\Bigr\}.\nonumber
        \end{align}
\end{proposition}

Before we present our closed-form solution to the above Gaussian optimization problem, let's first recall the optimal affine solution to the Witsenhausen counterexample, which is the same as in Witsenhausen's original paper \cite{witsenhausen1968}:

\begin{lemma}[\!\!\protect{\cite[Lemma 11]{witsenhausen1968}}, \protect{\cite[Lemma 5]{Treust2024power}}]
    The best linear policy is $U_1=-\sqrt{\frac{P}{Q}}X_0$, if $P\leq Q$, otherwise $U_1=-X_0 + \sqrt{P-Q}$, which induces the estimation cost
    \begin{align}
        S_{\ell}(P)=\begin{cases}\frac{(\sqrt{Q}-\sqrt{P})^{2}\cdot N}{(\sqrt{Q}-\sqrt{P})^{2}+N} & \text{ if } P\in[0,\ Q],\\ 0 &\text{ otherwise } .\end{cases}\label{eq: opt linear cost}
    \end{align}
\end{lemma}
The best linear cost provides an upper bound for the optimal Gaussian cost. However, the function $P\mapsto S_{\ell}(P)$ is not always convex. The estimation cost induced by the optimal joint Gaussian design summarized in Theorem \ref{thm: best gaussian policy} below obtains the convex envelope of $S_{\ell}$, which coincides with the solution proposed by Witsenhausen in \cite[Lemma 12]{witsenhausen1968} and the solution for the problem of flipped causality \cite[Theorem 2]{Treust2024power}. 

% \begin{theorem}[Optimal joint Gaussian cost for causal-noncausal setup]\label{thm: best gaussian policy}
%     The optimal Gaussian estimation cost for Witsenhausen problem with causal encoder and non-causal decoder is given by 
%     \begin{flalign} S_{\mathsf {G}}(P) =& \begin{cases} \frac {N\cdot (Q-N-P)}{Q} & \text {if } Q> 4N \text { and } P\in [P_{1},P_{2}],\\ S_{\ell }(P) & \text {otherwise. } \end{cases} \label{opt gaussian cost}\end{flalign}
%     where the parameters
%     \begin{align}
%         P_1 &= \frac{1}{2}(Q-2N-\sqrt{Q^2-4QN}),\label{eq: p1}\\
%         P_2 &= \frac{1}{2}(Q-2N+\sqrt{Q^2-4QN}).\label{eq: p2}
%     \end{align}
% \end{theorem}
In this theorem, $P_1$ and $P_2$ given in \eqref{eq: p1} and \eqref{eq: p2} are the two operating points for conducting the time-sharing strategy, which enables us to achieve a cost gain from the affine policy.


The following lemma states the general relation of Gaussian covariance coefficients given a Markov chain. It is a direct consequence combining several well-known results.


% We first present the following lemma, which is derived directly from known results, and states the general relation of Gaussian covariance coefficients given a Markov chain.
% % The proof of Theorem \ref{thm: best gaussian policy}, Lemma \ref{lemma: markov-covariance} and Corollary \ref{cor: causal cost with feedback} are shown in the Appendix.

% \begin{lemma}\label{lemma: markov-covariance}
%     If the jointly Gaussian random vector $(X,Y,Z)$ satisfy the Markov chain $X -\!\!\!\!\minuso\!\!\!\!- Y -\!\!\!\!\minuso\!\!\!\!- Z$ and have a covariance matrix
%     \begin{align}
%         \Sigma_{X,Y,Z} = \begin{pmatrix}
%             P & \rho_1\sqrt{PQ} & \rho_2\sqrt{PV}\\
%             \rho_1\sqrt{PQ} & Q &\rho_3\sqrt{QV}\\
%             \rho_2\sqrt{PV}&\rho_3\sqrt{QV} & V
%         \end{pmatrix},\label{eq: cov xyz}
%     \end{align}
%     with the covariance coefficients $(\rho_1,\rho_2,\rho_3)\in[-1,1]^3$ ensuring that $\det\brackets{\Sigma_{X,Y,Z}}\geq 0$, then, we have
%     \begin{align}
%         \rho_2=\rho_1\rho_3.\label{eq: rho_2=rho_1rho_3}
%     \end{align}
    
% \end{lemma}

% In other words, with the context of the Markov chain of jointly Gaussian $X -\!\!\!\!\minuso\!\!\!\!- Y -\!\!\!\!\minuso\!\!\!\!- Z$, if $X$ and $Y$ (or if $Z$ and $Y$) are uncorrelated (i.e., if $\rho_1=0$ or $\rho_3=0$), it follows that $X$ and $Z$ are also uncorrelated (i.e., $\rho_2=0$).


\begin{corollary}\label{cor: causal cost with feedback}
    The setup for causal encoder and non-causal decoder with channel feedback (i.e., channel output $Y_1$ is available to the first DM) has the same cost result \eqref{opt gaussian cost}.
\end{corollary}

The cost region characterization of this setup is investigated in \cite[Sec. C]{zhao2024causal}. From Corollary \ref{cor: causal cost with feedback}, we get that having channel feedback information to assist communication does not contribute to any performance gain in the Gaussian case.

Moreover, we recall Witsenhausen's two-point strategy proposed in \cite{witsenhausen1968}, and here, we refer it to \textit{one-step strategy}. It outperforms the best Gaussian cost \eqref{opt gaussian cost} for some values of $Q$ and $N$.
\begin{theorem}[\protect{\cite[Theorem 2]{witsenhausen1968}}]\label{thm: Witsenhausen 2-point}
    For parameter $a\geq 0$, Witsenhausen's one-step strategy is given by
    \begin{align}
        U_1 = a\cdot \mathsf{sign}(X_0) - X_0. \label{eq: two-point}
    \end{align}
    The power and estimation costs are given by
    \begin{align}
        P_1(a) &= Q + a\brackets{a - 2\sqrt{\frac{2Q}{\pi}}},\\
        S_1(a) &= a^2\sqrt{\frac{2\pi}{N}}\phi\brackets{\frac{a}{\sqrt{N}}}\int \frac{\phi\brackets{\frac{y_1}{\sqrt{N}}}}{\cosh{(\frac{ay_1}{N})}}dy_1,
    \end{align}
    where $\phi(x) = \frac{1}{\sqrt{2\pi}}e^{-\frac{x^2}{2}}$ and the optimal receiver's strategy is given by $\mathbb E\big[X_1\big|Y_1 = y_1\big]=a\tanh{(\frac{ay_1}{N})}$.
\end{theorem}

The core idea of the one-step strategy is to cancel the continuous source state $X_0$, such that the encoder designates the system state $X_1=U_1+X_0=a\cdot \mathsf{sign}(X_0)$ to be a perfect one-step function, i.e., a binary symbol, making it easier for the decoder to estimate.


% The numerical results of the best affine cost $S_\ell(P)$ in \eqref{eq: opt linear cost}, the optimal Gaussian cost $S_{\mathsf{G}}(P)$ in \eqref{opt gaussian cost} and Witsenhausen's one-step strategy cost $S_2(P)$ in \eqref{eq: two-point cost P} and \eqref{eq: two-point cost S} are illustrated in Fig \ref{fig: joint gaussian cost}, for the parameters $(Q,N)=(1, 0.15)$.
%     \begin{figure}[t]
%         \centering
%         \input{fig/joint Gaussian performance}
%         \caption{Comparison of the four cost functions $S_\ell(P)$, $S_{\mathsf{G}}(P)$, $S_2(P)$ and $S_{\mathsf{dpc}}(P)$. In this particular case, $S_2(P)$ outperforms $S_{\mathsf{G}}(P)$ and $S_\ell(P)$ when $P$ is above a certain level. }
%         \label{fig: joint gaussian cost}
%     \end{figure}


\begin{remark}Now, we discuss the optimal Gaussian cost for the case where both \ac{dm}s are causal.
\begin{itemize}
    \item The optimal Gaussian strategy discussed in \cite[App. B-B]{Treust2024power} is a single-letter (causal) approach, which provides a valid control strategy for a more restrictive setup assuming that the second \ac{dm} is also causal.  Therefore, \eqref{opt gaussian cost} is an upper bound of this cost. 
    \item From the genie-aided argument, a lower bound for the optimal cost is given by the optimal cost of a more superior system, such as the setup discussed in Corollary \ref{cor: causal cost with feedback}. Therefore, \eqref{opt gaussian cost} is a lower bound of the optimal cost of causal encoding and causal decoding Witsenhausen setup. 
\end{itemize}
Consequently, the optimal Gaussian cost for the causal encoding and decoding setup is also \eqref{opt gaussian cost}.
\end{remark}
    
    
    \begin{remark}\label{rmk: uniform Gaussian}
Our discussions above lead us to a remarkable conclusion: Even though the optimal achievable cost regions are different, the optimal Gaussian costs for the following five distinct configurations are the same:
    \begin{enumerate}
        \item Causal encoding and causal decoding.
        \item Causal encoding and non-causal decoding.
        \item Causal encoding and non-causal decoding with channel feedback.
        \item Non-causal encoding and causal decoding.
        \item Non-causal encoding and causal decoding with source feedforward.
    \end{enumerate}
    This equality is surprising since these settings all have different single-letter optimal regions, but these regions coincide if we restrict to Gaussian schemes. Therefore, when considering causal DMs, we need to jump out of the joint Gaussian constraint.
\end{remark}


==> sections/temp.tex <==
\indent The goal is to find the  parameters $(V_1,a)$ that minimize the power cost, i.e. that are optimal for the following  problem.
\begin{align}
&\min   \qquad  V_1 + \brackets{Q+a^2-2a\sqrt{\frac{2Q}{\pi}}}\\
&\text{s.t.} \quad h(Y_1) - \frac{1}{2}\log_2(2\pi eN) - 1\geq 0.
\end{align}

Therefore, for a fixed power cost $P\geq 0$, $V_1$ is uniquely determined by the parameter $a$ which needs to satisfy the following condition
\begin{align}
    V_1 = P - \brackets{Q+a^2-2a\sqrt{\frac{2Q}{\pi}}}\geq 0.\label{eq: coord2 power cost constraint}
\end{align}





Since there is no closed form for the entropy of Gaussian mixture distributions, methods discussed in \cite{huber2008entropy, kim2015entropy} can be employed for numerical simulation.

We denote the set of parameters $a\geq 0$ that satisfy the power cost constraint \eqref{eq: coord2 power cost constraint} and the information constraint \eqref{eq: coord2 info constraint} by
\begin{align}
    \mathcal{A}_{\mathsf{ZEC}^{(1)}}(P) &= \{a\geq 0: h(Y_1)- \frac{1}{2}\log_2(2\pi eN) \geq 1, \label{eq: admissible set}
\\
    &\quad\quad \text{and }
    V_1 = P - \brackets{Q + a^2 - 2a\sqrt{\frac{2Q}{\pi}}}\geq 0 \}.\nonumber \end{align}


Based on the above derivation, the optimal cost function for the ZEC system is summerized in the following theorem:
\begin{theorem}\label{thm: zec}
   Given the power cost $P\geq 0$, the \ac{mmse} estimation cost for the one-step ZEC coding scheme \eqref{eq: ZEC-1 scheme} is given by
    \begin{align}
        S_{\mathsf{ZEC}^{(1)}}(P) = 0, \text{ for  }P\geq P_{\mathsf{ZEC}^{(1)}}^*, \label{eq: cost function lossless}
    \end{align}
    where the value  
\begin{align}
    P_{\mathsf{ZEC}^{(1)}}^* = \min\{ P: \mathcal{A}_{\mathsf{ZEC}^{(1)}}(P) \neq\varnothing\}.\label{eq: P^*}
\end{align}

\end{theorem}

